Ferromagnetic domains in the large-$U$ Hubbard model with a few holes: an FCIQMC study

Two-dimensional Hubbard lattices with two or three holes are investigated as a function of $U$ in the large-$U$ limit. In the so-called Nagaoka limit (one-hole system at infinite $U$), it is known that the Hubbard model exhibits a ferromagnetic ground-state. Here, by means of exact FCIQMC simulations applied to periodic lattices up to 24 sites, we compute spin-spin correlation functions as a function of increasing $U$. The correlation functions clearly demonstrate the onset of ferromagnetic domains, centred on individual holes. The overall total spin of the wavefunctions remain the lowest possible (0, or $\frac{1}{2}$, depending on the number of holes). The ferromagnetic domains appear at interaction strengths comparable to the critical interaction strengths of the Nagaoka transition in finite systems with strictly one hole. The existence of such ferromagnetic domains is the signature of Nagaoka physics in Hubbard systems with a small (but greater than one) number of holes.

==> newcommands.tex <==
% for some strange reason I also need this package here:
\usepackage{colortbl}

% 
% % redefine \textmu to other mu commands usefull inside text
% \renewcommand{\textmu}{$\upmu$}

% % redefine \textmu to other mu commands usefull inside text
% \renewcommand{\textmu}{$\upmu$}
\newcommand{\bacc}{Projektpraktikum}
%\newcommand{\bacc}{Bachelorarbeit}
% Caption with defined width
\newcommand{\wcaption}[2]{%
   \begin{minipage}{#1}%
   \caption{#2}%
   \end{minipage}%
}

\newcommand{\figureref}[1]{(Abbildung \ref{#1})}%
\newcommand{\eqnref}[1]{~(\ref{#1})}%

% Command for margin text with usefull style
%\newcommand{\marginlabel}[1]{\mbox{}\marginline{\hspace{0pt}\footnotesize\sffamily #1}}%
\newcommand{\marginlabel}[1]{\marginnote{#1}}%

%\newcommand{\comment}[1]{\marginnote{#1}}%

% Enable space for figures that extent into the margin (right and/or leftside)
% Can be used inside a figure
% Note: sidecap defines a similar environment 'wide' !
\newenvironment{widespace}[2]{%
   \begin{list}{}{%
      \setlength{\topsep}{0pt}%
      \setlength{\leftmargin}{#1}%
      \setlength{\rightmargin}{#2}%
      \setlength{\listparindent}{\parindent}%
      \setlength{\itemindent}{\parskip}%
   }%
   \item[]%
}%
{%
   \end{list}%
}%

\newlength{\marginwidth}
\setlength{\marginwidth}{\marginparwidth}
\addtolength{\marginwidth}{\marginparsep}

%% Beispiel:
% \begin{figure}
% \begin{widespace}{-\marginwidth}{0pt}
%  \subfloat[Bergzebrastute]
%  {\includegraphics[width=0.45\linewidth]{../Bilder/Eingewoehnung2.jpg}}
%  \hspace*{1em}
%  \subfloat[Morro Moco]
%  {\includegraphics[width=0.45\linewidth]{../Bilder/bergzebra2.jpg}}
% \end{widespace}
% \end{figure}


% quantum optics - Latex Commands: Math **********************************
% ------------------------------------------------------------------------
% by: Matthias Pospiech
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% --| Math |-------------------------------------------------------

% -- Replacements --
\newcommand{\comp}{\ast}
%\renewcommand{\dagger}{+}


% -- new commands --
\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\Abs}[1]{\left\lvert#1\right\rvert}
\providecommand{\norm}[1]{\left\Vert#1\right\Vert}
\providecommand{\Trace}[1]{\ensuremath{\Tr\{\,#1\,\}}} % Trace /Spur
%

% -- differentials --
\newcommand{\der}{\partial\mspace{2mu}} % partial diff
\newcommand{\td}{\,\mathrm{d}}	% total diff
\newcommand{\ddt}[1]{\frac{\td #1}{\td t}}

% -- Abbrevitations --
\renewcommand{\Re}{\text{Re}}			% Real value
\renewcommand{\Im}{\text{Im}}			% Real value
\newcommand{\complex}{\mathbb{C}} % Complex
\newcommand{\real}{\mathbb{R}}    % Real
%\newcommand{\R}{\real}						% Real
%\newcommand{\N}{\mathbb{N}}
%\newcommand{\Z}{\mathbb{Z}}
%\renewcommand{\L}{\mathcal{L}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\R}{\mathcal{R}}
%
\newcommand{\Ham}{\mathcal{H}}    % Hamilton
\newcommand{\Prob}{\mathscr{P}}    % Hamilton
\newcommand{\unity}{\mathds{1}}   % Real
%

\newcommand\gammab{\gamma_\bot}
\newcommand\gammap{\gamma_\parallel}
\newcommand\gammai{\gamma_\text{int}}
\newcommand\gammae{\gamma_\text{ext}}

% -- New Operators --
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\grad}{grad}
%\DeclareMathOperator{\div}{div}
\renewcommand{\div}{\text{div}\,}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\e}{e} 			% exponatial Function

% -- new symbols --
\newcommand{\laplace}{\Delta}
\newcommand{\dalembert}{\Box}

% -- new arrows --
\renewcommand{\leadsto}{\Longrightarrow}
\newcommand{\leftrightleadsto}{\Longleftrightarrow}


% -- Text subscripts--
\newcommand{\rel}{_\text{rel}}
%\newcommand{\st}{\text{st}}
%

% -- other --
\newcommand{\com}[2]{\underbrace{#1}_{\textrm{\scriptsize #2}}}
\newcommand{\with}[1]{\stackrel{\ref{#1}}{\Longrightarrow}}
%\newcommand{\unit}[1]{\,\textrm{#1}}

%\newcommand{\variance}[1]{\delta \mean{#1}^2}
\newcommand{\variance}[1]{(\Delta{#1})^2}
%\newcommand{\variance}[1]{\delta #1^2}

% -- Physics --------------------------------
\newcommand\op[1]{{\hat{\mathrm{#1}}}}  % Operator

%
%
\newcommand{\mean}[1]{\ensuremath{\overline{#1}}} % mean value
%
% \newcommand{\state}[1]{\ensuremath{\ket{#1}}}
%
\newcommand\commutator[2]{\ensuremath{\mathinner{%
    \mathopen[\,#1,#2\,\mathclose]}}}
\newcommand{\Commutator}[2]{\ensuremath{\left[\,#1,#2\,\right]}}
\newcommand{\bigcommutator}[2]{\ensuremath{\bigl[\,#1,#2\,\bigr]}}
\newcommand{\Bigcommutator}[2]{\ensuremath{\Bigl[\,#1,#2\,\Bigr]}}
%
\newcommand\poisson[2]{\mathinner{%
    \mathopen\{#1,#2\mathclose\}}}
%

% -- Layout --------------------------------

\newcommand*{\dashfill}{\leavevmode\cleaders\hbox{-}\hfill\kern0pt}

\newcommand*{\midhrulefill}{
\leavevmode
\cleaders\hbox to 1ex{\raisebox{.5ex}{\rule{1ex}{.4pt}}}\hfill\kern0pt
}

% evertz useful newcommands
% must be equal:
\newcommand{\mbeq}{\overset{!}{=}}
\newcommand{\mustbe}{\stackrel{!}{=}}

% bra - ket
% \newcommand{\ket}[1]{{\left| #1 \right>}}
% \newcommand{\bra}[1]{{\left< #1 \right|}}
\newcommand{\bracket}[2]{{\left\langle \vphantom{#1 #2} #1 \,\right|
  \left.\hspace{-0.15em} \vphantom{#1 #2} #2\right\rangle}}

\newcommand*{\braopket}[3]{\ensuremath{\langle{#1}|{#2}|{#3}\rangle}}

%\newcommand{\bigket}[1]{{\big| #1 \big>}}
%\newcommand{\bigbra}[1]{{\big< #1 \big|}}
%\newcommand{\Bigket}[1]{{\Big| #1 \Big>}}
%\newcommand{\Bigbra}[1]{{\Big< #1 \Big|}}
%
%% Def. Zahlenräume R,C,N
%\newcommand{\Rs}{\mathbb{R}}
%\newcommand{\Cs}{\mathbb{C}}
%\newcommand{\Ns}{\mathbb{N}}
%\newcommand{\Op}[1]{$\Hat{#1}$}

%order:
%\newcommand{\ordl}{{\cal O}(\lambda)}
%\newcommand{\ordll}{{\cal O}(\lambda^2)}
%%\newcommand{\ordlll}{{\cal O}(\lambda^3)}
%\newcommand{\orde}{{\cal O}(\epsilon)}
%\newcommand{\ordee}{{\cal O}(\epsilon^2)}
%\newcommand{\ordeee}{{\cal O}(\epsilon^3)}

% shortcuts
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\renewcommand{\d}{\downarrow}
\renewcommand{\u}{\uparrow}
\newcommand{\s}{\sigma}
%\renewcommand{\l}{\lambda}
% creation and annihilation ops
\renewcommand{\c}[2]{c_{#1,#2}}
\newcommand{\cd}[2]{c^\dagger_{#1,#2}}
\newcommand{\entspricht}{\mathop{\hat{=}}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\us}{$\u$-spin \,}
\newcommand{\ds}{$\d$-spin \,}
\newcommand{\Hd}{\hat{H}_\d}
\newcommand{\Hu}{\hat{H}_\u}
\newcommand{\n}[1]{n_{i,#1}}
\newcommand\expect[1]{\ensuremath{\left\langle{#1}\right\rangle}} 
\newcommand{\fig}[1]{fig.(\ref{#1})}
\newcommand{\G}{\Gamma}
\renewcommand{\P}{\mathcal{P}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\Var}{\text{Var}}
\newcommand{\sign}{\text{sign}}
\newcommand{\intsum}{\int\!\!\!\!\!\!\!\!\!\;\sum}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
%\renewcommand{\text}{\text}

% code environment: 
\def\code#1{\texttt{\detokenize{#1}}}
\def\c#1{\code{#1}}

% various stuff
\newcommand{\neci}{\texttt{NECI}}

% math columns: 
\newcolumntype{L}{>{$}l<{$}} % math-mode version of "l" column type
\newcolumntype{C}{>{$}c<{$}} % math-mode version of "l" column type

% specific colors 
%\definecolor{MPIgreen}{RGB}{0 129 112}
%\newcommand\crule[3][MPIgreen]{\textcolor{#1}{\rule{#2}{#3}}}

% /
\def\ul#1{\underline{#1}}
\def\ol#1{\overline{#1}}

\newcommand{\oL}{\ensuremath{\overline{L}}}
\newcommand{\oR}{\ensuremath{\overline{R}}}
\newcommand{\uL}{\ensuremath{\underline{L}}}
\newcommand{\uR}{\ensuremath{\underline{R}}}

\newcommand{\oLL}{\oL\oL}
\newcommand{\oRR}{\oR\oR}

\newcommand{\uLL}{\uL\uL}
\newcommand{\uRR}{\uR\uR}

\newcommand{\oRL}{\oR\oL}
\newcommand{\uRL}{\uR\uL}

\newcommand{\ra}{\ensuremath{\rightarrow}}
\newcommand{\la}{\leftarrow}

\newcommand{\q}{\quad}
\newcommand{\D}{\Delta}

%\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
%\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\def\bigO#1{\mathcal{O}(#1)}

% different vector: 
%\renewcommand*{\v}[1]{\ensuremath{\mathbf{#1}}}

\newcommand{\myuparrow}{\color{red}$\u$}
\newcommand{\mydownarrow}{\color{blue}$\d$}
%\newcommand{\red}{\color{red}}
%\newcommand{\todo}[1]{\emph{\smaller\color{red}{(todo:#1)}}}

%\newcommand*{\citen}{}% generate error, if `\citen` is already in use
%\DeclareRobustCommand*{\citen}[1]{%
%  \begingroup
%    \romannumeral-`\x % remove space at the beginning of \setcitestyle
%    \setcitestyle{numbers}%
%    \cite{#1}%
%  \endgroup
%}
\newcommand{\diffp}[2]{\frac{\partial#1}{\partial#2}}

%\newcommand{\botrule}{\bottomrule}

==> standard_packages.tex <==

% some standard packages I almost always use!

% decide between those 2:
%\usepackage[utf8]{inputenc}
\usepackage[english]{babel}

\usepackage{etex}
%\usepackage{default}

% i hope there is no conflict between thos color packages! 
\usepackage{graphicx}
\usepackage{color}
\usepackage{colortbl}
\usepackage{xcolor}
\usepackage{calc}

% math symbols! 
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{wasysym}

\usepackage{float}
\usepackage{epstopdf}
%\usepackage{esdiff}
\usepackage{nicefrac}

\usepackage{tcolorbox}% http://ctan.org/pkg/tcolorbox
\usepackage{marvosym}

\usepackage[makeroom]{cancel}

% have to think about which subfigure stuff i want to use! 
%\usepackage{subfigure}
%\usepackage{subfig}

% \usepackage{subcaption}

% different young tableau packages: 
\usepackage[vcentermath]{youngtab} % for Young tableaux
%\usepackage{young} % for Young tableaux
%\usepackage{ytableau}

% TIKZ:
\usepackage{tikz}
%\usepackage{tikz-qtree}

\usetikzlibrary{trees}
\usetikzlibrary{calc}
\usetikzlibrary{positioning}
% here is a conflict with some other package:
%\usetikzlibrary{tikzmark,decorations.pathreplacing,shapes.misc}
%\usetikzlibrary{tikzmark}%,decorations.pathreplacing,shapes.misc}
\usetikzlibrary{shapes.misc}
\usetikzlibrary{decorations.pathreplacing}

\usetikzlibrary{shapes.arrows} 
\usetikzlibrary{backgrounds}

\tikzset{
  solid node/.style = {circle, draw, inner sep = 3, fill = black},
  right angle/.style = {grow = 300},
  left angle/.style = {grow = 240},
  short/.style = {level distance = 1cm, },
  long/.style = {level distance = 2cm},
  left up/.style = {grow = 120},
  right up/.style = {grow = 60}
}

\usepackage{rotating}
% math-tools also conflicts with some other package!
\usepackage{mathtools}
\usepackage{hyperref}

\usepackage{units}
% this also conflicts with some other package!
\usepackage{tabularx}
\usepackage{booktabs}
\usepackage{pgf}
\usepackage{pgfplots}
\usepackage{geometry}
%\usepackage{longtable}
%\usepackage{floatrow}
\usetikzlibrary{calc,intersections}
\usepackage{relsize}
\usepackage{longtable}

%Options: Sonny, Lenny, Glenn, Conny, Rejne, Bjarne, Bjornstrup
%\usepackage[Sonny]{fncychap}
\usepackage{dcolumn}
\usepackage{braket}
% for posting code snippets:
\usepackage{listings}
% or choose: algorithmic, algorithm2e, algorithmicx(algpseudocode), and program
% or \usepackage{algorithm}
%\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{relsize}
\usepackage{nicefrac}
\usepackage{mathdots}

\usepackage{diagbox}

\usepackage{standalone}
%\draft % marks overfull lines with a black rule on the right

\usepackage{bm}% bold math
\usepackage{multirow}

% choose between 1 of them:
\usepackage{acronym}
%\usepackage{glossaries}

\usepackage{tikzorbital}
\usepackage{sidecap}

\usepackage{setspace}
\usepackage{bbold}
\pgfplotsset{compat=newest}


==> tikz_styles.tex <==
\definecolor{spawncolor}{RGB}{200 0 0}
\definecolor{deathcolor}{RGB}{0 200 0}
\definecolor{annihilcolor}{RGB}{255 99 71}
\definecolor{endcolor}{RGB}{255 99 71}

% special tikz node styles for the CI states:
\tikzset{state node/.style={circle,thick,inner sep=1pt}}

% state connections
\tikzset{state conn/.style={very thick}}
\tikzset{state dash/.style={very thick, dashed}}

% walker "weights"
\tikzset{walker/.style={very thick}}
\tikzset{walker new/.style={very thick, red}}
\tikzset{spawn/.style={very thick, color=spawncolor}}
\tikzset{death/.style={very thick, color=deathcolor}}
\tikzset{annihil/.style={very thick, color=annihilcolor}}
% new length to seperate the states
\newlength{\shortlength}
\setlength{\shortlength}{1cm}
\newlength{\longlength}
\setlength{\longlength}{2cm}

\newlength{\afourwidth}
\setlength{\afourwidth}{21cm}

% and the "walker occupation"
\newlength{\walkerlength}
\setlength{\walkerlength}{0.5cm}

\newlength{\tablesep}
\setlength{\tablesep}{0.3cm}

\newlength{\gridsep}
\setlength{\gridsep}{1cm}

% x-axis node style

\tikzset{branch/.style={circle,draw,thick,inner sep=1pt}}
\tikzset{growd/.style={-,very thick, red}}
\tikzset{grid/.style={-}}

\tikzset{lattline/.style={-,thick}}

\newlength{\orbsep}
\setlength{\orbsep}{0.5cm}

\newlength{\sepone}
\setlength{\sepone}{0.5cm}

\newlength{\septwo}
\setlength{\septwo}{1cm}

\newlength{\septhree}
\setlength{\septhree}{1.5cm}

\tikzset{graph/.style={circle,draw,thick,inner sep=2pt}}
\tikzset{graphline/.style={-,thick}}

\tikzset{site/.style={circle,very thick,draw,opacity=0.8,inner sep=1pt}}

\newlength{\latticesep}
\setlength{\latticesep}{0.5cm}

\newlength{\indicator}
\setlength{\indicator}{1cm}

\tikzset{orbline/.style={-,very thick}}

\tikzset{doubspin/.style={-,very thick}}
\tikzset{posspin/.style={-,very thick,blue}}
\tikzset{negspin/.style={-,very thick,red}}

\newlength{\picsep}
\setlength{\picsep}{3cm}

\newlength{\stepzero}
\setlength{\stepzero}{1cm}
\tikzset{loop-tail/.style={circle,thick,inner sep=1pt,draw,fill}}
\tikzset{tree-out/.style={circle,thick,inner sep=1pt,draw,fill}}

\tikzset{mline/.style={thick}}

\newlength{\onedist}
\setlength{\onedist}{0.5cm}

\newlength{\twodist}
\setlength{\twodist}{2\onedist}

\newlength{\threedist}
\setlength{\threedist}{3\onedist}

\tikzset{inter/.style={circle,thick,inner sep=1pt,draw}}
\tikzset{mprime/.style={thick,dashed}}

\newlength{\taildist}
\setlength{\taildist}{2.5cm}

\newlength{\headdist}
\setlength{\headdist}{5cm}

\tikzset{line-out/.style={thick,dotted}}

\newlength{\gridlen}
\setlength{\gridlen}{5cm}

\tikzset{drt-vert/.style={circle,very thick,draw}}

\tikzset{tree-start/.style={rectangle,very thick,draw,rounded corners=2pt,text width = {width("1")}, text height = {height("1")}, outer sep = 0,inner sep = 4pt}}%, outer sep = 0, inner sep = 1pt, align=center}}
\tikzset{tree-mid/.style={circle,very thick, draw,  text width = {width("1")}, text height = {height("1")}, outer sep = 0, inner sep = 2pt,align=center}}

\definecolor{csf-color-1}{RGB}{0 200 0}
\definecolor{csf-color-2}{RGB}{255 99 71}

%\tikzset{fixed-node/.style={circle,very thick, draw, minimum width = {width("1")},align = center, minimum height = {\heightof("1")}}}

\tikzset{fixed-node/.style={circle,very thick, draw,  text width = {width("10")}, text height = {height("10")}, outer sep = 0, inner sep = 1pt,align=center}}

\tikzset{empty-node/.style={circle,very thick,  text width = {width("10")}, text height = {height("10")}, outer sep = 0, inner sep = 1pt,align=center}}

%\tikzset{empty-node/.style={circle,very thick, align=center, text width = {width("10")}}}

\definecolor{doublecolor}{RGB}{200 0 0}
\definecolor{singlecolor}{RGB}{0 200 0}

\tikzset{lattline/.style={-,thick}}
\tikzset{fermi/.style={rounded corners}}
\tikzset{line/.style={very thick}}
\tikzset{arrow/.style={->,very thick}}
\tikzset{box/.style={fill=white,rounded corners=1pt, opacity = 0.95, text opacity = 1.0}}

\tikzset{gridline/.style={dashed,opacity = 0.2}, very thin}

\definecolor{navyblue}{RGB}{0 0 128}
\definecolor{cadetblue}{RGB}{95 158 160}
\definecolor{branchingcolor}{RGB}{210 105 30}

\definecolor{back_fill}{gray}{0.9}
\definecolor{back_fill_dark}{gray}{0.7}

\tikzset{end-node/.style = {tree-out, ,text width = 2pt,text height = 2pt}}

\tikzset{l-long/.style= {<-,thick,out = 315, in = 45}}
\tikzset{r-long/.style= {->,thick,out = 315, in = 45}}

\tikzset{l-short/.style= {<-,thick,out = 315, in = 45}}
\tikzset{r-short/.style= {->,thick,out = 315, in = 45}}
\tikzset{bubble/.style= {->,thick,out = 340, in = 20}}
\tikzset{bubble-left/.style= {->,thick,out = 225, in = 110}}

\tikzset{r-long-left/.style= {->,thick,out = 225, in = 135}}
\tikzset{l-long-left/.style= {<-,thick,out = 225, in = 135}}
\tikzset{r-short-left/.style= {->,thick,out = 225, in = 135}}
\tikzset{l-short-left/.style= {<-,thick,out = 225, in = 135}}

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\tikzset{flow-box/.style={rectangle,very thick,draw,rounded corners=2pt}}%, outer sep = 0, inner sep = 1pt, align=center}}

\tikzset{flow-box-end/.style={rectangle,very thick,draw,rounded corners=2pt}, draw = red}%, outer sep = 0, inner sep = 1pt, align=center}}
\tikzset{flow-arrow/.style={->,very thick,rounded corners}}
